Gain variations as induced by the diffuse night sky background: the ASTRI-Horn experience

ASTRI-Horn is the prototype of the nine telescopes that form the ASTRI Mini-Array, under construction at the Teide Observatory in Tenerife (Spain), devoted to observe the sky in the 1--200 TeV energy band. It adopts an innovative optical design based on a dual-mirror Schwarzschild-Couder configuration, and the camera, composed by a matrix of monolithic multipixel silicon photomultipliers (SiPMs) is managed by ad-hoc tailored front-end electronics based on a peak-detector operation mode. During the Crab Nebula campaign in 2018-2019, ASTRI-Horn was affected by gain variations induced by high levels of night sky background. This paper reports the work performed to detect and quantify the effects of these gain variations in shower images. The analysis requested the use of simultaneous observations of the night sky background flux in the wavelength band 300-650 nm performed with the auxiliary instrument UVscope, a calibrated multi-anode photomultiplier working in single counting mode. As results, a maximum gain reduction of 15% was observed, in agreement with the value previously computed from the variance of the night sky background level in each image. This ASTRI-Horn gain reduction was caused by current limitation of the voltage supply. The analysis presented in this paper provides a method to evaluate possible variations in the nominal response of SiPMs when scientific observations are performed in the presence of high night sky background as in moon conditions.

==> conclusion.tex <==
\section{Summary and conclusion}
\label{sect:conclusion}
In this paper we presented results on the evaluation of the gain variation that affected the fast signal detected by ASTRI-Horn in correlation with the increase of the NSB flux. These results were compared with those obtained by the analysis of the event background as presented in our  previous work \cite{Compagnino2022} and we found that data were affected by a maximum gain variation of $\sim$15\%, and that the the values measured with from the background and fro the signal are compatible within errors.
The analysis was performed using a set of data collected during the Crab Nebula campaign on December 2018. 

The good quantitative agreement between the two approaches clearly distinguish two level of efficiency of the ASTRI Camera, where to a given flux value of about 5625 ph m$^{-2}$ ns$^{-1}$ sr$^{-1}$, 
the gain reduction reaches a maximum value of about 14\%.\\
These methods of analysis are useful diagnostic tools able to evaluate the gain uniformity of the whole focal plane
during scientific observations.\\
The limit in the PDM power system of ASTRI-Horn was updated in an version optimized to greatly alleviate the problem of
the gain loss.\\
Moreover, an upgraded version of the power system able to supply a constant power up to 12 times the current level
will be implemented in the cameras being designed for the ASTRI-MA telescopes.


